Mapping high-performance RNNs to in-memory neuromorphic chips

The increasing need for compact and low-power computing solutions for machine learning applications has triggered significant interest in energy-efficient neuromorphic systems. However, most of these architectures rely on spiking neural networks, which typically perform poorly compared to their non-spiking counterparts in terms of accuracy. In this paper, we propose a new adaptive spiking neuron model that can be abstracted as a low-pass filter. This abstraction enables faster and better training of spiking networks using back-propagation, without simulating spikes. We show that this model dramatically improves the inference performance of a recurrent neural network and validate it with three complex spatio-temporal learning tasks: the temporal addition task, the temporal copying task, and a spoken-phrase recognition task. We estimate at least 500x higher energy-efficiency using our models on compatible neuromorphic chips in comparison to Cortex-M4, a popular embedded microprocessor.

==> source/mismatch_sims50.tex <==
\begin{adjustbox}{center}
\begin{tabular}{@{}lrrrrr|rrrrr@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Layer}} & \multicolumn{5}{c}{$\mu_{NMSE}$}                                                          & \multicolumn{5}{c}{$\sigma_{NMSE}$}                                                           \\ \cmidrule(l){2-11} 
\multicolumn{1}{c}{}                       & $c_{v_p}$  = 0 & $c_{v_p}$  = 0.2 & $c_{v_p}$  = 1 & $c_{v_p}$  = 1.5 & $c_{v_p}$  = 2 & $c_{v_p}$  = 0 & $c_{v_p}$  = 0.2 & $c_{v_p}$  = 1 & $c_{v_p}$  = 1.5 & $c_{v_p}$  = 2 \\ \midrule
% Input Dense layer              & 1.0           & 1.0             & 1.0           & 1.0            & 1.0           & 0.0           & 0.0             & 0.0           & 0.0             & 0.0           \\
Recurrent layer 1              & 1.0           & 1.0             & 0.3           & 0.4            & -1.3          & 0.1           & 0.1             & 2.0           & 2.1             & 7.4           \\
% Dense layer 1                  & 1.0           & 1.0             & 0.0           & 0.1            & -2.2          & 0.2           & 0.1             & 2.5           & 3.1             & 7.1           \\
Recurrent layer 2              & 0.9           & 0.7             & -1.2          & -7.4           & -5.9          & 0.2           & 0.3             & 3.5           & 15.5            & 13.1          \\
% Dense layer 2                  & 0.9           & 0.7             & -2.1          & -7.5           & -11.1         & 0.2           & 0.4             & 4.6           & 15.3            & 26.8          \\
Recurrent layer 3              & 0.8           & -0.1            & -17.5         & -32.6          & -21.0         & 0.4           & 1.5             & 42.6          & 89.1            & 25.6          \\
% Dense layer 3                  & 0.9           & 0.2             & -4.5          & -14.7          & -10.7         & 0.2           & 0.8             & 5.7           & 34.9            & 12.1          \\
Recurrent layer 4              & 0.9           & -1.3            & -33.9         & -123.5         & -61.7         & 0.2           & 4.5             & 98.8          & 407.6           & 102.0         \\
% Output Dense layer             & 0.9           & 0.1             & -7.1          & -33.4          & -19.5         & 0.2           & 1.0             & 7.5           & 75.1            & 28.1          
\\ \bottomrule
\end{tabular}
\end{adjustbox}
